TRACE: Intra-visit Clinical Event Nowcasting via Effective Patient Trajectory Encoding

Electronic Health Records (EHR) have become a valuable resource for a wide range of predictive tasks in healthcare. However, existing approaches have largely focused on inter-visit event predictions, overlooking the importance of intra-visit nowcasting, which provides prompt clinical insights during an ongoing patient visit. To address this gap, we introduce the task of laboratory measurement prediction within a hospital visit. We study the laboratory data that, however, remained underexplored in previous work. We propose TRACE, a Transformer-based model designed for clinical event nowcasting by encoding patient trajectories. TRACE effectively handles long sequences and captures temporal dependencies through a novel timestamp embedding that integrates decay properties and periodic patterns of data. Additionally, we introduce a smoothed mask for denoising, improving the robustness of the model. Experiments on two large-scale electronic health record datasets demonstrate that the proposed model significantly outperforms previous methods, highlighting its potential for improving patient care through more accurate laboratory measurement nowcasting. The code is available at https://github.com/Amehi/TRACE.

==> related.tex <==

\section{Related Works}
In recent years, deep learning has made significant progress in the healthcare domain, particularly through its application to electronic health records (EHR). Models driven by advanced neural networks have shown substantial promise across a range of clinical tasks, mainly including mortality prediction \cite{suresh_learning_2018, tan_data-gru_2020, jiang2023graphcare, cai_cohortnet_2024}, risk prediction \cite{choi_gram_2017, ma_risk_2018, choi_mime_2018, zhang_grasp_2021}, diagnosis prediction \cite{ma_dipole_2017, bai_interpretable_2018,ma_kame_2018, lee_diagnosis_2018, choi_mime_2018, gao_camp_2019}, and medication recommendation \cite{zhang_leap_2017, wang_order-free_2019, tan_4sdrug_2022}. Despite differences in these tasks, their core objective is to derive representations of patients' health status \cite{zhang_grasp_2021}. To the best of our knowledge, all prior works have concentrated on visit-level representations, where models make predictions for the next patient visit based on historical data. In this paper, we address clinical predictions within every singular patient visit.

\subsection{\textbf{Mortality Prediction \& Risk Prediction}} Mortality prediction estimates a patient’s likelihood of death within a specific time frame, while risk prediction assesses the probability of future adverse events, such as disease onset. Despite their different focuses, both are formulated as binary classification tasks.
% Recurrent neural network (RNN), including long short-term memory (LSTM) \cite{hochreiter1997long} and gated recurrent units (GRU) \cite{Cho_2014}, are widely used to process sequential data in EHR applications. 

Recurrent neural networks (RNNs), known for their ability to process sequential data, are widely used to model patient trajectories in EHR data. RETAIN \cite{choi_retain_2016} is an interpretable model for binary prediction tasks that applies two RNNs with attention mechanisms to capture visit-level and medical code-level importance. StageNet \cite{gao_stagenet_2020} designs a stage-aware long short-term memory (LSTM) module to extract the disease progression stages and integrates a convolutional module that leverages stage information to improve predictive accuracy. With the advancement of Natural Language Processing (NLP) technologies, the Transformer model emerged and has rapidly become a popular choice for handling sequential input data due to its efficiency and effectiveness. HiTANET \cite{luo_hitanet_2020} uses a Transformer model with a time-aware attention mechanism, combining local visit-level and global time-step attention to improve risk prediction. Some works explore the predictive power of laboratory measurements in EHR data. ConCare \cite{ma_concare_2019} utilizes a multi-channel GRU to model the different laboratory features of patients. Similarly, AdaCare \cite{ma_adacare_2020} employs a GRU-based architecture with dilated convolutions to capture long-term and short-term variations in laboratory biomarkers. In this work, we also highlight the critical role of laboratory data within EHR records and design a model specifically for the task of predicting future laboratory measurements, instead of only using them as the input.

\subsection{\textbf{Diagnosis Prediction \& Medication Recommendation}}Both diagnosis prediction and medication recommendation are formulated as multi-label classification tasks. Cohort learning has emerged as a growing trend, effectively enhancing model inference by capturing shared patterns and relationships within patient groups. GRASP \cite{zhang_grasp_2021} uses the K-Means algorithm to cluster patient embeddings, which supports the learning of cohort representations and the extraction of knowledge from patient groups. Meanwhile, many studies have demonstrated the effectiveness of graph-based techniques in improving performance on these tasks. GRAM \cite{choi_gram_2017} constructs an ontology graph from the intrinsic information of medical codes, enabling interpretable representation learning. Building on the approach used in GRAM, KAME \cite{ma_kame_2018} enhances the model's reasoning ability by exploiting the category-level information of input medical events with a more general knowledge graph. GAMENet \cite{shang_gamenet_2019} employs graph-augmented memory networks to model the intricate relationships between medications, and MoleRec \cite{yang_molerec_2023} introduces a substructure-aware molecular representation learning approach to improve combinational drug recommendation. GraphCare \cite{jiang2023graphcare} constructs patient-specific and medical concept-specific knowledge graphs to facilitate downstream prediction tasks. 
These works usually incorporate external domain knowledge via graph-based techniques, while our approach does not rely on such extra information.
% While these works integrate external domain knowledge using graph-based techniques to enhance their models, our approach does not rely on such external knowledge.

% TRANS \cite{chen2024trans} models patients' EHR data as a temporal heterogeneous graph, effectively capturing both graph-structured and temporal relationships between different medical events.
% Core \cite{liu_toward_2023} propose a novel 
% A recent study CohortNet \cite{cai_cohortnet_2024} advances cohort discovery for interpretable healthcare analytics by using graph-based methods and attention mechanisms to identify and analyze patient cohorts.

% \textbf{Mortality Prediction}. Mortality prediction has been a crucial task in healthcare, with many studies utilizing electronic health records (EHR) to forecast patient outcomes. For instance, AdaCare \cite{} leverages scale-adaptive clinical feature extraction to improve both interpretability and prediction accuracy of the model.\\
% \textbf{Risk Prediction}. Risk prediction, aimed at detecting the likelihood of future adverse events such as disease onset or deterioration, is another key area where EHR data is widely utilized.\\
% \textbf{Diagnose Prediction}. Accurate diagnostic prediction is foundational to effective treatment and patient care, with sequential models increasingly being applied to EHR data for this purpose.\\
% \textbf{Medication Recommendation} Medication recommendation is a highly specialized task that requires an understanding of both the patient’s medical history and the complex interactions between different drugs.\\

